3D-aware Image Generation and Editing with Multi-modal Conditions

3D-consistent image generation from a single 2D semantic label is an important and challenging research topic in computer graphics and computer vision. Although some related works have made great progress in this field, most of the existing methods suffer from poor disentanglement performance of shape and appearance, and lack multi-modal control. In this paper, we propose a novel end-to-end 3D-aware image generation and editing model incorporating multiple types of conditional inputs, including pure noise, text and reference image. On the one hand, we dive into the latent space of 3D Generative Adversarial Networks (GANs) and propose a novel disentanglement strategy to separate appearance features from shape features during the generation process. On the other hand, we propose a unified framework for flexible image generation and editing tasks with multi-modal conditions. Our method can generate diverse images with distinct noises, edit the attribute through a text description and conduct style transfer by giving a reference RGB image. Extensive experiments demonstrate that the proposed method outperforms alternative approaches both qualitatively and quantitatively on image generation and editing.

==> 6_ack.tex <==
We are grateful to Google University Relationship GCP Credit Program for the support of this work by providing computational resources.

==> fig_baselines.tex <==
\begin{figure*}[t]
\centering
\includegraphics[width=\textwidth]{compare.png}
 \vspace{-2em}
\captionof{figure}{
\textbf{Qualitative Comparison with Pix2Pix3D\cite{deng20233d}, SoFGAN\cite{chen2021sofgan}, and SEAN\cite{zhu2020sean}} on CelebAMask dataset. Pix2pix3d fails to maintain texture information. SEAN fails in multi-view synthesis, while SoFGAN suffers from multi-view inconsistency (e.g., face identity changes across viewpoints). Our method renders high-quality images while maintaining multi-view consistency. Please check our \href{http://cs.cmu.edu/~pix2pix3D}{website} for more examples.
}


\vspace{-1em}
\lblfig{seg2face_baselines}
\end{figure*}

==> fig_edge_cat.tex <==
\begin{figure}[t!]
    \centering
    \includegraphics[width=\linewidth]{edge_cat.pdf}
    \vspace{-2em}
    \caption{\looseness=-1 Conditional generation with edge map and reference image as conditions.
    % The first column is the input edge map, the first row is the input image, the generated geometry feature of each row is determined by the same edge map. Our method can maintain good geometry while implementing style transfer from input images and produce realistic multi-view results.  %
    }
    \label{fig:edge_cat}
    \vspace{-0.5em}
\end{figure}

==> fig_method.tex <==
\begin{figure*}[h!]
    \centering
    \includegraphics[width=\linewidth]{fig_method_small2.pdf}
    \vspace{-2em}
    \caption{\looseness=-1\textbf{Overall pipeline.} Given a 2D label map (e.g., segmentation map), a random latent code $z$, and a camera pose $\hat P$ as inputs, our generator renders the label map and image from viewpoint $\hat P$. Intuitively, the input label map specifies the geometric structure, while the latent code captures the appearance, such as hair color. We begin with an encoder that encodes both the input label map and the latent code into style vectors $\mathbf{w}^{+}$. We then use $\mathbf{w}^{+}$ to modulate our 3D representation, which takes a spatial point $\mathbf{x}$ and outputs (1) color $\mathbf{c}\in \mathbb{R}^3$, (2) density $\sigma$, (3) feature $\phi \in \mathbb{R}^{l}$, and (4) label $\mathbf{s} \in \mathbb{R}^{c}$. We then perform volumetric rendering and 2D upsampling to get the high-res label map $\mathbf{\hat I}_{\mathbf{s}}^+$ and RGB Image $\mathbf{\hat I}_{\mathbf{c}}^+$. For those rendered from ground-truth poses, we compare them to ground-truth labels and images with an LPIPS loss and label reconstruction loss. We apply a GAN loss on labels and images rendered from both novel and original viewpoints. %
    }
    \lblfig{method}
    \vspace{-0.5em}
\end{figure*}

==> fig_text_beard.tex <==
\begin{figure}[h!]
    \centering
    \includegraphics[width=\linewidth]{text_beard.pdf}
    \vspace{-2em}
    \caption{\looseness=-1\textbf{Text editing on beard attribute}  %
    }
    \label{fig:text_beard}
    \vspace{-0.5em}
\end{figure}

==> tab_ablation.tex <==
\begin{table}[h]
\setlength{\tabcolsep}{2pt}
% \setlength{\extrarowheight}{3pt}
\renewcommand{\arraystretch}{0.8}
\centering
\scriptsize
\begin{tabular}{lccc}
\toprule
  & \multicolumn{2}{c}{\textsc{Quality}} & \multicolumn{1}{c}{\textsc{Identity}} \\ %
& & &  \\

\textsc{CelebAMask\cite{CelebAMask-HQ}} & FID $\downarrow$  & KID $\downarrow$ & ID $\downarrow$  \\ 
\midrule
\textsc{w/o Attention } & 18.97 & 0.007 & 1.125 \\
\textsc{w/ Attention } & 21.28 & 0.008 & \textbf{0.978} \\
\bottomrule
\end{tabular}
\caption{\textbf{Ablation Study on Attention Module.} In order to explore the impact of the attention module on the degree of texture-geometry decoupling, we randomly selected 5k style codes and two different semantic maps for each style code, calculated the similarity of the generated faces by same style code. }
\vspace{-1em}

\label{table:ablation}
\end{table}
